MEMA Runtime Framework: Minimizing External Memory Accesses for TinyML on Microcontrollers

We present the MEMA framework for the easy and quick derivation of efficient inference runtimes that minimize external memory accesses for matrix multiplication on TinyML systems. The framework accounts for hardware resource constraints and problem sizes in analytically determining optimized schedules and kernels that minimize memory accesses. MEMA provides a solution to a well-known problem in the current practice, that is, optimal schedules tend to be found only through a time consuming and heuristic search of a large scheduling space. We compare the performance of runtimes derived from MEMA to existing state-of-the-art libraries on ARM-based TinyML systems. For example, for neural network benchmarks on the ARM Cortex-M4, we achieve up to a 1.8x speedup and 44% energy reduction over CMSIS-NN.

==> tables/dlmc_table.tex <==
\begin{table}[ht]
\centering
 \caption{$M \times K \times N$ Dimension of Layers in DLMC Benchmark}
  \label{tab:terms}
 \centering
 \scalebox{1}{
\begin{tabular}{ c l }
\hline
Layer Id & Dimension \\% inserts table %heading
\hline % inserts single horizontal line
1 & $512\times2048\times256$ \\
2 & $512\times512\times256$ \\
3 & $2048\times512\times256$ \\
4 & $512\times2048\times512$ \\
5 & $512\times512\times512$ \\
6 & $2048\times512\times512$ \\
7 & $512\times2048\times1024$ \\
8 & $512\times512\times1024$ \\
9 & $2048\times512\times1024$ \\
10 & $512\times2048\times2048$ \\
11 & $512\times512\times2048$ \\
12 & $2048\times512\times2048$ \\
\hline % inserts single horizontal line
\end{tabular}
}
\end{table}

==> tables/terms_table.tex <==
\begin{table}[ht]
\centering
 \caption{Terminology used throughout the paper}
  \label{tab:terms}
 \centering
 \scalebox{1}{
\begin{tabular}{ c l }
\hline
Term & Description \\% inserts table %heading
\hline % inserts single horizontal line
 AI & Arithmetic Intensity \\ 
 CT & Computation Throughput\\
 IO & \# of Operands Transferred for Memory Access\\ %Input and Output
 MB & Memory Bandwidth\\
 MCU & Microcontroller \\
 MM & Matrix-Matrix Multiplication \\ 
 Tile & Sub-matrix \\
\hline % inserts single horizontal line
\end{tabular}
}
\end{table}



==> tables/tiny_table.tex <==
\begin{table}[ht]
\centering
 \caption{$M\times K \times N$ Dimension of Layers in MLPerf Tiny Benchmark}
  \label{tab:terms}
 \centering
 \scalebox{1}{
\begin{tabular}{ c l }
\hline
Layer Id & Dimension \\% inserts table %heading
\hline % inserts single horizontal line
1 & $16\times27\times1024$ \\
2 & $16\times144\times1024$ \\
3 & $32\times144\times256$ \\
4 & $32\times288\times256$ \\
5 & $32\times16\times256$ \\
6 & $64\times288\times64$ \\
7 & $64\times576\times64$ \\
8 & $64\times32\times64$ \\
9 & $64\times40\times122$ \\
10 & $64\times64\times125$ \\
11 & $8\times27\times2304$ \\
12 & $16\times8\times2304$ \\
13 & $32\times16\times576$ \\
14 & $32\times32\times576$ \\
15 & $64\times32\times144$ \\
16 & $64\times64\times144$ \\
17 & $128\times64\times36$ \\
18 & $128\times128\times36$ \\
19 & $256\times128\times9$ \\
20 & $256\times256\times9$ \\
\hline % inserts single horizontal line
\end{tabular}
}
\end{table}


\scalebox{0.66}{
 \begin{tabular}{ c l }
\hline
Layer Id & Dimension \\% inserts table %heading
\hline % inserts single horizontal line
11 & $8\times27\times2304$ \\
12 & $16\times8\times2304$ \\
13 & $32\times16\times576$ \\
14 & $32\times32\times576$ \\
15 & $64\times32\times144$ \\
16 & $64\times64\times144$ \\
17 & $128\times64\times36$ \\
18 & $128\times128\times36$ \\
19 & $256\times128\times9$ \\
20 & $256\times256\times9$ \\
\hline % inserts single horizontal line
\\ \\
\end{tabular}
}
